Decision-Focused Evaluation: Analyzing Performance of Deployed Restless Multi-Arm Bandits

Restless multi-arm bandits (RMABs) is a popular decision-theoretic framework that has been used to model real-world sequential decision making problems in public health, wildlife conservation, communication systems, and beyond. Deployed RMAB systems typically operate in two stages: the first predicts the unknown parameters defining the RMAB instance, and the second employs an optimization algorithm to solve the constructed RMAB instance. In this work we provide and analyze the results from a first-of-its-kind deployment of an RMAB system in public health domain, aimed at improving maternal and child health. Our analysis is focused towards understanding the relationship between prediction accuracy and overall performance of deployed RMAB systems. This is crucial for determining the value of investing in improving predictive accuracy towards improving the final system performance, and is useful for diagnosing, monitoring deployed RMAB systems. Using real-world data from our deployed RMAB system, we demonstrate that an improvement in overall prediction accuracy may even be accompanied by a degradation in the performance of RMAB system -- a broad investment of resources to improve overall prediction accuracy may not yield expected results. Following this, we develop decision-focused evaluation metrics to evaluate the predictive component and show that it is better at explaining (both empirically and theoretically) the overall performance of a deployed RMAB system.

==> AI4SG Workshop (AAAI 23) Submission/ARMMAN_real_world_studies.tex <==
\section{Real-World ARMMAN studies}
\label{section:previous_studies}

% Points to elaborate:\\

% -- In this section we summarize the performance of our original RMAB-based system in the real-world studies we performed.

% \noindent
% -- Our RMAB-based system will be compared only to the control baseline and not to RR for the subsequent analysis, as our analysis to explain better performance of RR over RMAB was inconclusive, however, we do have sufficient empirical evidence to justify the better performance of RMAB in Apr 21 as compared to the other two studies. We would possibly show 1) the engagement drops prevented graphs, or just the number of active beneficiaries over time.

% \noindent
% -- In this section we would conclude that RMAB performed best in Apr 21, its performance was worst in Jan 22, and in May 22 as well it didn't perform well, however it was better than Jan 22.

The first real-world study in which RMAB system was deployed in the context of ARMMAN was performed by Mate et al. in April 2021. This study tracks a cohort of 23000 beneficiaries for 7 weeks. The cohort was divided into three groups -- round robin, RMAB and the current standard of care (CSOC). In every group, 125 beneficiaries were selected for intervention every week. In the round robin group, beneficiaries are given service call on a first-come first serve basis based on their registration date. In the RMAB group, beneficiaries are chosen for service calls using the Whittle index policy. The current standard of care group received no service call. The study demonstrated that the RMAB-based system resulted in a $\sim30\%$ reduction in the engagement drops as compared to CSOC group.

To rigorously check the efficacy of the RMAB model, several subsequent field tests have been performed. Specifically, we performed two followup studies where different training datasets are used to learn the mapping function from beneficiaries' demographic data to the MDP parameters; the training dataset in the context of ARMMAN simply comprises of (i) the beneficiaries' socio-demographic features, and (ii) their observed transition data from a past field study. In the April 2021 study, a training dataset used to learn the demographic features to the MDP parameter mapping was collected in a study performed in May 2020 where an RMAB system wasn't used to plan the interventions. 
The second study was performed in  January 2022 using a cohort of 44,000 beneficiaries and it went on for $5$ weeks wherein in each week, in each group, 250 beneficiaries were chosen for intervention. The demographic features to transition probability mapping was learnt using trajectories of beneficiaries' behaviour observed in the April 2021 Study, i.e., the training dataset for January 2022 study was April 2021. In the third study, which was performed in May 2022, the data from the January 2022 study was used for training; it tracked a cohort of 15,000 beneficiaries and the budget of intervention each week was 175. The RMAB system performed very well in the April 2021 study -- resulting in more than ~$30\%$ reduction in the engagement drops as compared to the CSOC baseline.
Figure \ref{fig:studies} shows the cumulative engagement drops prevented by RMAB system as compared to the CSOC group adjusted by the number of service calls.
% However, in the subsequent two studies, a similar performance wasn't observed. That is,
Clearly, a consistent performance of the RMAB system is not observed across the 3 studies, with April 2021 study performing the best, followed by May 2022 and January 2022 studies wherein the cumulative engagement drops prevented by RMAB system weren't significant.
% the performance of the RMAB-based system was much worse in the May 2022, January 2022 study as compared to the April 2021 study. 
Given this, the goal of the current work is to diagnose and identify the right evaluation method through which we can explain the different performance of the RMAB model across the three studies.

\begin{figure}
    \centering
    \includegraphics[width=0.7\columnwidth]{3studies.png}
    \caption{Performance of the RMAB system across the three studies}
    \label{fig:studies}
\end{figure}


==> AI4SG Workshop (AAAI 23) Submission/conclusion.tex <==
\section{Conclusion}

First we demonstrated that the prediction accuracy analysis alone is insufficient and inconclusive in understanding the  performance of RMAB systems --- this was demonstrated using real-world data of an RMAB system deployed in the context of a maternal health awareness program together with a NGO. We then proposed a decision-focused evaluation method for RMAB systems and showed that this is a far more meaningful evalution to establish correlation with the real-world performance of the RMAB system. Notably, our work primarily focused on RMAB systems, solved using the Whittle index approach. We believe that this analysis will be useful for other deployed applications of RMAB in other domains as well. 

%This new method of evaluation was based on analyzing the errors in computing the top-k Whittle indices.

% Identifying whether the phenomenon we identified --- prediction accuracy not correlating with the real-world performance --- also occurs in domains where the optimization algorithm is not RMAB would be an interesting direction of future research. %Additionally, in our analysis we used clustering to address the issue of lack of data to estimate all the transition probabilities; we used k-means towards the same. Having a systematic method of performing this data imputation -- comparing and contrasting different clustering approaches would also be interesting.



% This new method of evaluation is motivated by the fact the just analysing the performance of RMAB-based system based on the accuracy of predicting the transition probabilities can be misleading, this was demonstrated using the real-world data of the ARMMAN NGO. 

%Following a decision-focused approach, we compared several methods of defining the errors in computing top Whittle indices. 
% Finally, the decision-focused evaluation method was used on the real-world data of ARMMAN NGO and we showed that it is indeed able to explain the real-world performance of RMAB system.


==> AI4SG Workshop (AAAI 23) Submission/introduction.tex <==
\section{Introduction}  % and Paritosh]}

Restless Multi Armed Bandits (RMABs) is a general framework for solving sequential decision making problems and has been employed in a wide variety of application domains such as planning preventive interventions for healthcare ~\cite{mate2022field}, anti-poaching patrols \cite{QianRestlessPoachers}, communication systems~\cite{Liu2010,liu2012learning}, sensor monitoring tasks~\cite{glazebrook2006indexable}, etc.
Most of the works on RMAB have focused on studying the optimization problem of allocating limited resources, assuming perfect knowledge of the underlying parameters of the RMAB model \cite{bertsimas2000restless,nino2001restless,verloop2016asymptotically,mate2020collapsing}. As a result, RMABs have seen limited deployment in practice, especially in applications such as healthcare and conservation where the RMAB parameters of the agents being catered to, are unknown in the real-world. 
% However, their real world application have been challinging due to limited avialablility of transition probability parameters. 
Existing approaches that implement RMAB solutions to resource allocation problems typically adopt a two-staged, predict-then-optimize framework \cite{wang2020restless,osband2013more,jung2019regret,mate2022field}. In the first stage, these approaches learn a machine learning model that predicts the necessary RMAB parameters and then in the second stage, solve the RMAB optimization problem using these predictions. 
% This pushed RMAB problems into a predict-then-optimize framework where we first predict the required parameters and then solve the optimization problem.


We pose the question of understanding the relationship between prediction accuracy and overall RMAB system performance. Such an understanding is important for two reasons. First, we want to understand if investing in improved prediction accuracy warrants improved system performance. Second, once an RMAB-based system is deployed in the real-world, we are interested in monitoring its performance and providing diagnosis to understand the potential sources of improvements in the data-to-deployment pipeline.  In general, we expect that if the RMAB model parameters are accurately predicted, the system's decisions are indeed guaranteed to be optimal; similarly, we expect that given a fixed optimization engine, higher overall prediction accuracy would lead to improved RMAB performance.

%However, one challenge in such RMAB systems is the evaluation of its efficacy in the real world. Specifically, having seen the results of the implemented solution, we address the question of how to diagnose the deployment and understand potential sources of improvements in the data-to-deployment pipeline. Given a fixed optimization engine, it would seem that the more accurate the prediction of the parameters in an RMAB system, the better the result. 

\paragraph{Our contributions.} \emph{Our first contribution is to show, using for the first time an RMAB system deployed in the public health domain, that improving machine learning prediction accuracy alone -- particularly measured using standard measures of error like RMSE or MAE -- may not lead to improved overall system performance. In fact there may be a degradation in performance.} Evaluating the performance of RMABs in context of a real-world deployment (described below), we demonstrate this important phenomenon, and as our second contribution propose an alternative, decision-focused evaluation approach of the machine learning component to address this issue. Broadly speaking, a key take away lesson of our work is that instead of investing resources including compute, data or human resources for broad improvements in prediction accuracy, our proposed decision-focused evaluation metrics may provide a better guide for investment in RMAB deployment. Moreover, many systems deployed in the real-world follow a two-staged, predict-then-optimize framework \cite{ford2015beware,fang2016deploying,perrault2019ai}, our work highlights that even in these domains we shouldn't directly assume, or design systems based on a correlation between prediction accuracy and overall performance. 

We demonstrate our results and describe the methodological contributions via one such application of the predict-then-optimize framework for RMABs. %We dissect this real world application of RMABs and analyze results.
We collaborate with ARMMAN, an Indian NGO, that aims to improve access to maternal health information in underprivileged communities. Through their flagship program mMitra, ARMMAN delivers critical health information to new and expectant mothers via automated phone calls. However, the engagement rates among mMitra's beneficiaries dwindle over time and as a fix, ARMMAN delivers live service calls to encourage engagement. Due to limited resources, only a small fraction of beneficiaries can be selected for live service calls every week. This is cast as an RMAB problem where we must decide which beneficiaries to choose every week for live service calls. 
% We adopt the Whittle index based solution strategy --- the dominant solution strategy for RMABs --- for determining which beneficiaries to pick each week for service calls. 

Using our proposed decision-focused evaluation approach for RMABs, we analyze the performance of RMAB-based system deployed for ARMMAN, i.e., all our analysis is based on real-world data where decisions concerning real individuals were taken via an RMAB. The deployed RMAB system employs the Whittle index based method ---  which is the most prominent solution concept for RMABs. We compare and contrast different methods of defining errors in top-k Whittle indices. As our final contribution in this paper, we show that an error definition based on the Spearman's footrule measure \cite{diaconis1977spearman}\footnote{Spearman's footrule is used to quantify the disarray between two permutations} is best suited in this context for decision-focused evaluation. Our proposed approach is indeed able to predict the real-world performance of our RMAB system better than prediction accuracy analysis.



==> AI4SG Workshop (AAAI 23) Submission/methodology.tex <==
\section{Methodology} % [Paritosh]}

The key idea that underlies the analysis is to use the transition data of the beneficiaries observed in the real-world as the ground truth i.e., as a basis of our analysis. Specifically, the observational data reflects the \emph{true} transition probabilities of the arms (beneficiaries) which, ideally-speaking should have been the basis of our decisions. However, as described next, the limited amount of observational data presents itself as a major challenge here.

\paragraph{Computing Missing Observed Transition Probabilities via Clustering.} The observed transitions of each beneficiary $i$ forms an sequence $\langle (s, a, s') \rangle$, where $(s, a, s')$ denotes that the beneficiary $i$ transitioned from the state $s$ to state $s'$ under action $a$ in a particular week; here $s,s',a \in \{0,1\}$. From the observed transitions we can empirically estimate the true transition probabilities of each arm. However, due to the limited number of active interventions, we do not have sufficient observed data to estimate all the transition probabilities for each beneficiary. In particular, the amount of active transition probabilities are limited because most of the beneficiaries (more than $80\%$) do not receive even a single service call during the entire study, due to which we cannot empirically estimate their true active transition probabilities; however, for most beneficiaries, we have sufficient observational data to estimate the passive transition probabilities.

To compute the missing transition probabilities we (i) cluster the beneficiaries based on their observed passive transition probabilities, then (ii) for each resulting cluster, we pool the observed transitions of all the beneficiaries in that cluster, this ensures that we have sufficient data to compute active transition probabilities for each cluster. Then, (iii) the missing active transition probabilities of each beneficiary is assigned to be the active transition probability of the cluster in which that beneficiary lies. This procedure enables us to compute the missing observed transition probabilities.  

Once the missing observed transition probabilities are inferred using the described method, we analyze the errors in predicting transition probabilities. However, we show that the prediction errors are insufficient in explaining the real-world performance. This motivates us to pursue an alternate, more decision-focused evaluation approach. The decision-focused analysis is based on evaluating the errors in computing the top Whittle indices, which is in line with the Whittle index policy. Towards this, we compare/contrast different methods of computing the Whittle indices and show that a definition based on the well-known Spearman's footrule distance~\cite{diaconis1977spearman} is best suited in this context. Using this, we analyze the performance of the RMAB system deployed in the context of ARMMAN. To get a deeper understanding of the performance, we also present a probabilistic analysis to quantify how well is our RMAB system performing as compared to a purely random algorithm as per the proposed metric.

% of ARMMAN, with the expected value and standard deviation of errors had we used a purely random algorithm to select beneficiaries for intervention. This analysis gives us information as to how much better is our RMAB-based algorithm performing as compared to a purely random algorithm. 

% The prediction accuracy analysis is presented in the next section (Section \ref{section:transition_probability_errors}), and the decision-focused analysis is detailed in Section \ref{section:decision_focused_analysis}.

% Points to elaborate:

% \noindent
% -- Method of imputing missing transition probabilities: k-means on passive probabilities, and pooling active transitions; mostly all the active transition probabilities are missing. Associated assumptions "beneficiaries having similar passive transition probabilities have similar active transition probabilities"

% \noindent
% -- Mention that in the next section (or either in the appendix) we evaluate the impact of imputing the missing transition probabilities and show that the comparison of errors across the three studies remains the same even if we do the error analysis without imputation.

==> AI4SG Workshop (AAAI 23) Submission/preliminaries.tex <==
\section{Preliminaries}


\paragraph{Restless Multi-Armed Bandits}
The RMAB framework is characterized by $N$ independent Markov Decision Processes \cite{mdp-puterman}, which are referred to as arms. Each arm is represented by a 4-tuple $\{\mathcal{S}, \mathcal{A}, R, \mathcal{P}\}$. $\mathcal{S}$ denotes the state space,  which could be a good state "beneficiary adhering to the program" or bad state "beneficiary not adhering to the program". $\mathcal{A}$ is the set of possible actions which we consider to be binary in our case, i.e., an action could be active, pulling an arm; or passive, not pulling an arm.  $R$ is the reward function $R: \mathcal{S} \times \mathcal{A} \times \mathcal{S} \rightarrow \mathbb{R}$. And $P$ denotes the probability of transitioning to the next state $s' \in \mathcal{S}$ starting from a current state $s \in \mathcal{S}$ under action $a \in \mathcal{A}$. We denote this probability as $P(s, a, s')$. The policy $\pi$ for an arm is defined as the mapping $\pi : \mathcal{S} \rightarrow \mathcal{A}$, i.e., it dictates the action to be taken given the current state. The objective that we maximize in the RMAB framework is sum of expected discounted rewards for all arms. For a single arm having a starting state $s_0$, this reward can be written as $V_{\beta}^\pi(s_0) = \mathbb{E}\left[\sum_{t=0}^\infty \beta^tR(s_t, \pi (s_t), s_{t+1}|\pi, s_0)\right]$. The next state are drawn from the distribution $s_{t+1} \sim P(s_{t}, {\pi(s_t)}, s_{t+1})$ where $\beta \in [0,1)$ is called the discount factor and $P$ represents the transition probabilities of that arm.
% The expected \emph{discounted reward} starting from state $s_0$ is defined as $V_{\beta}^\pi(s_0) = \mathbb{E}\left[\sum_{t=0}^\infty \beta^tR(s_t, \pi (s_t), s_{t+1}|\pi, s_0)\right]$ where the next state is drawn according to $s_{t+1} \sim P_{s_t,s_{t+1}}^{\pi(s_t)}$,  $\beta \in [0,1)$ is the discount factor and actions are selected according to the policy mapping $\pi$. 
% % \hl{The \emph{average reward} $\overline{V}^\pi$ of policy $\pi$ is defined as the expected reward computed over the occupancy frequency: $\overline{V}^\pi = \sum_{s \in \mathcal{S}} x^\pi(s) R(s)$, where $x^\pi(s)$ denotes the average fraction of time spent in the state $s$.} 
% The planner's goal is to maximize the total reward. 
% The state value function $V^{\pi} (s_t)$ is then defined as the expected return starting from the state $s_t$ and following the policy $\pi$. Similarly, the action value function $Q^{\pi} (s_t, a_t)$ is defined as the expected return starting from $s_t$, taking the action $a_t$ and following the policy $\pi$.



% We model the engagement behavior of each beneficiary by an MDP corresponding to an arm of the RMAB. Pulling an arm corresponds to an active action, i.e., making a service call (denoted by $\alpha=a$), while $\alpha=p$ denotes the passive action of abstaining from a call. The state space $\mathcal{S}$ consists of binary valued states, $s$, that account for the recent engagement behavior of the beneficiary; $s \in [NE,E]$ (or equivalently, $s \in [0,1]$) where $E$ and $NE$ denote the `Engaging' and `Not Engaging' states respectively. For example, in our domain, \textbf{ABC} considers that if a beneficiary stays on the automated voice message for more than 30 seconds (average message length is 1 minute), then the beneficiary has engaged. If a beneficiary engages at least once with the automated voice messages sent during a week, they are assigned the engaging ($E$) state for that time step and non-engaging ($NE$) state otherwise.

% For each action $\alpha \in \mathcal{A}$, the beneficiary states follow a Markov chain represented by the 2-state Gilbert-Elliot model \cite{gilbert1960capacity} with transition parameters given by $P_{ss'}^\alpha$, as shown in Figure~\ref{fig:MDP}. With slight abuse of notation, the reward function $R(.)$ of $n^{th}$ MDP is simply given by $R_n(s)=s$ for $s \in \{0,1\}$. 



% Computing the optimal policy for an RMAB is PSPACE-hard. Whittle \cite{whittle-rbs}, proposed an index-based heuristic, known today as the Whittle Index, that can be solved in polynomial time. It has been shown to be asymptotically optimal for the time average reward problem \cite{weber1990index} and other families of RMABs arising from stochastic scheduling problems \cite{glazebrook2006indexable}.
% The Whittle Index technique operates by computing an index for every arm, which intuitively captures the value of pulling that arm. The Whittle approach considers each arm separately for the index computation, effectively decoupling the arms and converting it to $N$ smaller problems. The Whittle Index policy for the RMAB is to pull the $k$ arms with the highest 

Finding the optimal solution for RMAB problems is known to be PSPACE-hard \cite{papadimitriou1994complexity}. The Whittle Index policy \cite{whittle-rbs} is a computationally efficient heuristic for solving RMAB. The idea of Whittle Index is to provide a subsidy whenever the passive action is chosen by the planner. The value of the infimum subsidy such that there is no difference in choosing among active or passive actions is then defined as the Whittle Index. Specifically, $W(s)=inf_{\lambda}\{\lambda:Q_{\lambda}(s,a=0)=Q_{\lambda}(s,a=1)\}$ where $Q(s, a)$ is the $Q$-value or expected discounted future reward of taking an action $b$ from state $s$. The Whittle index policy operates by selecting $k$ beneficiaries having the highest Whittle indices in each decision step.

% We adopt the Whittle solution approach described previously for solving the RMAB. It hinges around the key idea of a ``passive subsidy'', which is a hypothetical reward offered to the planner, in addition to the original reward function for choosing the passive action. 
% % We use $Q_m^{\pi} (s_t, a_t)$ to denote the expected return starting from $s_t$, taking the action $a_t$ and following the policy $\pi$, when the passive subsidy offered is $m$. Intuitively,  higher the passive subsidy (denoted as $m$) offered, more attractive is the passive action to the planner.
% The Whittle Index is then defined as the infimum subsidy that makes the planner indifferent between the `active' and the `passive' actions, i.e.,:
% \begin{equation}
% W(s)=inf_{\lambda}\{\lambda:Q_{\lambda}(s,p)=Q_{\lambda}(s,a)\}    
% \end{equation}
% %However, this passive subsidy value is well-defined only if a technical condition called `indexability' is satisfied. 
% % In practice, Whittle index has proven to be a useful heuristic in many settings even when indexability has not been formally proven. We use a similar approach in this paper, and provide a proof of indexability ( here or in appendix?).
\paragraph{ARMMAN}
Beneficiaries are enrolled into ARMMAN's mMitra program by healthcare workers. These enrollments are either made at hospitals or through door-to-door surveys. At registration time, beneficiaries' socio-demographic information such as age, education, income, number of children, gestational age, etc is noted. Additionally, based on whether the beneficiaries have already delivered the baby or not, they are enrolled in the Antenatal Care or Postnatal Care program. Then automated voice calls with health information tailored according to the gestational age of the beneficiaries are sent; the duration of call listened to is stored in a database. Both the listenership data and the demographic information is stored in an anonymized manner.

The engagement behaviour of every beneficiary is modelled through an MDP. The binary valued actions correspond to making a service call (denoted by $a=1$, active action) or not making a service call (denoted by $a=0$, passive action); the action set $\mathcal{A} = \{0,1\}$. 
In the ARMMAN setting, we define the states of each beneficiary (arm) based on their recent engagement with the system. Specifically, if a beneficiary listens to at least one automated voice call with more than 30 seconds in a week, the beneficiary is marked as engaging. Thus, $s=0$, corresponds to Non-Engaging (NE) state and $s=1$ corresponds to Engaging (E) state; the set of states $\mathcal{S} = \{0,1\}$. Finally, with 2 states and 2 actions, the Markov chain for every beneficiary can be represented using a 2-state Gilbert-Elliot model \cite{gilbert1960capacity}. The reward function is chosen to maximize the engagement of beneficiaries (i.e., number of engaging beneficiaries) in the long run. Specifically, the reward function for the $n^{th}$ arm/beneficiary is simply defined to be, $R_n(s)=s$ for state $s \in \{0,1\}$.

==> AI4SG Workshop (AAAI 23) Submission/problem_statement.tex <==
\section{Problem Statement}% [Paritosh and Shresth]}

Our aim is to understand how prediction accuracy relates to the overall performance of a deployed RMAB system. This understanding is required to guide system improvements and is crucial for monitoring, diagnosing, and interpreting the performance of deployed RMAB system. One might expect to see improvement in performance following an improvement in prediction accuracy, thus prediction accuracy might seem to be a natural objective to steer the design of the overall RMAB system.

However, we show that simply improving the prediction accuracy for RMABs may not result in overall performance improvement, and therefore an alternate evaluation method is needed for RMAB systems. Moreover, there are multiple, seemingly-reasonable ways in which we can evaluate RMAB systems, and it is not immediately clear which is the most appropriate criterion. Consequently, our goal is to design a method of evaluating RMAB systems that correlates with and offers insights into the real-world performance, and additionally is versatile enough to enable analysis from various perspectives.


% This is motivated by the fact that RMABs can be used to model a wide variety of sequential decision making problems in various domains like security, wildlife conservation, public health, etc. 



% such that the decrease in error also gets reflected in improvement in the real-world performance. 
% In this work, we propose such a definition of errors in top-k Whittle indices. Additionally, using probabilistic analysis we give bounds on the expectation and the standard deviation of this error value, so that we can quantify how much better is the RMAB system performing as compared to a purely random policy.
% We pose the question of understanding the relationship between prediction accuracy  and overall RMAB system performance. This is critical for two reasons: First, it is useful to understand the value of investing on improving predictive accuracy towards improving the final system performance. Second, this understanding is instructive in monitoring and diagnosing the performance of a deployed RMAB system.  

% Towards facilitating this understanding, our contributions are as follows. First we provide and analyze the results from a first-of-its-kind deployment of RMABs. Second we illustrate that, counter to natural expectations, improved overall prediction accuracy does not lead to improvement in  the real-world performance of the RMAB system. Third, we present a decision-focused evaluation approach of the predictive component and show that it is better at explaining the performance of real-world RMAB system. Fourth we propose specific decision-focused evaluation metrics, which we hope would guide diagnosis of RMAB systems in the future.

==> AI4SG Workshop (AAAI 23) Submission/related_work.tex <==
\section{Related Work}
Sequential resource allocation problems arise in many real-world scenarios in healthcare domain.
%such as wildlife conservation \cite{QianRestlessPoachers,sodagari2011anti}, border patrol security \cite{klima2014online},  social engineering attacks \cite{miehling2018bayesian}, including public health. An important subclass of such problems are the sequential resource allocation problems where some limited resources are to be distributed over time to optimize for long term rewards.
For example, adherence monitoring is an extensively studied problem \cite{martin2005challenge} where the goal is to carefully allocate the limited number of available healthcare workers or resources to monitor and improve patients' adherence to medication for diseases like cardiac problems~\cite{corotto2013heart}, tuberculosis~\cite{Killian_2019, ong2014effects,chang2013house} and HIV~\cite{HIV}. These mentioned works largely focus on developing machine learning model to classify beneficiaries as high risk, or predict their future adherence patterns. However, these approaches essentially rely on making one-shot predictions and fail to capture the sequential aspect the of decision making needed to maximize long term rewards. Other works have also used reinforcement learning to design health monitors and provide personalized suggestions and notifications to users~\cite{liao2020personalized, pollack2002pearl}; notably, these works do not deal with the problem of allocating limited resources, as there is no constraint on the number of notifications being sent.



%This setting has been studied in multiple contexts such as green security games \cite{QianRestlessPoachers} where rangers are to be deployed in national parks to counteract poacher operations or for radio networks \cite{sodagari2011anti}. 
% In this context, often machine learning models are trained to use background information of beneficiaries and past adherence behaviour to predict future adherence patterns.
% One downside of such models is that they treat adherence problem as a single-shot prediction problem. However, such problems are inherently sequential and requires long term planning.

% Patient adherence monitoring in healthcare has been shown to be an important problem \cite{martin2005challenge}, and is closely related to the churn prediction problem, studied extensively in the context of industries like telecom \cite{dahiya2015customer}, finance \cite{XIE20095445, shaaban2012proposed}, etc.
% The problem of tracking agents' continued engagement with a system is known as Adherence Monitoring.
% Adherence monitoring is an extensively studied problem in healthcare \cite{martin2005challenge} with close ties to the problem of churn prediction in industries like finance \cite{XIE20095445,shaaban2012proposed}, telecom \cite{dahiya2015customer}, etc. 
% Another field that is closely related to Adherence Monitoring is that of Campaign Optimization where potential customers are to be reached out through phone calls.
% Past works have exploited the social network structure of customers \cite{Leskovec2007campaign} \cite{eagle2010network}, as well as behavioural and demographic features to find the set of customers who will improve the outreach of campaign. However, in our domain, having prior information on social network among beneficiaries is not feasible. 
% However, campaign optimization is also a single shot problem while in adherence setting, behaviour has to be optimized for multiple timesteps.

% Within healthcare, several studies have been conducted on Patient Adherence for diseases such as cardiac problems \cite{son2010application} \cite{corotto2013heart}, Tuberculosis \cite{Killian_2019} \cite{10.1001/archinte.1996.00440020063008}, HIV \cite{HIV} etc.

% In such studies, machine learning models are trained to use agents' background information and past adherence behaviour to predict future adherence patterns. One downside of such models is that they treat adherence problem as a single-shot prediction problem. However, adherence is a sequential problem and requires planning for optimizing long term adherence.

% Another shortcoming of such single-shot prediction models is that they can flag large number of patients as  high risk, while in a practical setting, only limited number of patients can be prioritized. 

% The healthcare domain has seen several studies on patient adherence for diseases like HIV \cite{HIV}, cardiac problems \cite{son2010application, corotto2013heart}, Tuberculosis \cite{Killian_2019, 10.1001/archinte.1996.00440020063008}, etc. These studies use a combination of patient background information and past adherence data, and build machine learning models to predict future adherence to prescribed medication.
% However, such models treat adherence monitoring as a single-shot problem and are unable to appropriately handle the sequential resource allocation problem at hand. 

% Additionally, the pool of beneficiaries flagged as high risk can itself be large, and the model can't be used to prioritize calls on a periodic basis, as required in our settings.




% Campaign optimization (via phone outreach) has also been studied previously. Most existing works \cite{Leskovec2007campaign, eagle2010network} however, rely on the availability of a customer social network based on  preferences, behavior or demographics, to help identify the set of key customers who will increase the reach of the campaign. In our domains of interest, %there is no detailed information of preferences that is available and more importantly, based on analysis done by our partner NGO, 
% there is no evidence of a social network among the beneficiaries, so such campaign optimization techniques are inapplicable. Furthermore, campaign optimization relies on single-shot interventions for optimization, whereas, our problem requires tracking progress of beneficiaries over multiple timesteps. 

% The Restless Multi-Armed Bandit (RMAB) framework has been popularly adopted to tackle such sequential resource allocation problems \cite{whittle-rbs} \cite{jung2019regret}. 


Restless Multi-Armed Bandit is a popular framework \cite{whittle-rbs,jung2019regret} used for solving sequential resource allocation problems that require long term planning. 
In an RMAB instance the decision choices/alternatives are represented by Markov Decision Processes (MDPs) which are in turn characterized by their transition dynamics.
% and captures the uncertainty associated with the particular decision choice. However, finding the optimal solution for RMAB problems is known to be PSPACE-hard. Whittle Index policy \cite{whittle-rbs} is one of the most prominent technique for solving RMAB. It is computationally efficient and in a time average reward setting, it is shown to be asymptotically optimal \cite{weber1990index}.
% The RMAB framework is also popular in many security games where sequential resource allocation has to be done to counteract over adversaries. In \cite{QianRestlessPoachers}, rangers are to be deployed in national parks to counteract poacher operations while in \cite{sodagari2011anti}, an anti-jamming strategy is formulated for radio networks. Broadly, bandit frameworks have been used in security games such as data poisoning attacks \cite{ma2018data}, border patrol security \cite{klima2014online}, social engineering attacks \cite{miehling2018bayesian} etc.
One major challenge in using RMABs in the real-world is the problem of unknown transition dynamics. Several previous works such as  \cite{LiuIndexRB,QianRestlessPoachers,mate2021risk} assume that transition dynamics are already known beforehand, making them unsuitable for real-world deployment.

% RMABs consist of $N$ independent Markov Decision Processes (MDPs), where each MDP models the transition dynamics of one specific beneficiary, and the subset of beneficiaries for intervention are selected according to their Whittle Indices \cite{whittle-rbs}. 
% Computing the optimal solution for RMAB problems is shown to be PSPACE-hard. Whittle proposed an index-based heuristic \cite{whittle-rbs}, that can be solved in polynomial time and is now the dominant technique used for solving RMABs. It has been shown to be asymptotically optimal for the time average reward problem \cite{weber1990index}, and other families of RMABs arising from stochastic scheduling problems \cite{glazebrook2006indexable}. Several works as listed in Section~\ref{sec:intro}, show applicability of RMABs in different domains 
% % \cite{LiuIndexRB, QianRestlessPoachers, mate2021risk} 
% but these unrealistically assume perfect knowledge of the RMAB parameters, and have not been tested in real-world contexts.

% \cite{arpitaijcai,avrachenkov2020whittle} propose a Whittle-Index Q-Learning approach to tackle the the unknown transition dynamics problem. But this technique is not sample-efficient and thus limited for real-world context.

% Another class of work leverages clustering to infer the transition dynamics with limited background data. In \cite{gentile2014onlin} \cite{li2019improved} \cite{yang2020exploring} \cite{li2021unifying}, clustering is used in the Multi-Armed bandits and contextual bandit problems.
% However, these works do not consider RMAB setting. 
A common approach is to estimate the transition dynamics by inferring them using background information.
% In \cite{mate2022field}, clustering for RMAB is performed on beneficiaries' past transition behaviours. Consequently, a predictive model is learnt to map the beneficiaries into one of the clusters using their socio-demographic features.
However, the predictive model learnt in such works maximizes the accuracy of predicting transition dynamics. This can create a mismatch between the objective being maximized and the final decision outcome. Such a mismatch can result in unintended consequences for the system, as highlighted in \cite{Boettiger_2022} in the context of fisheries management.

In contrast, decision-focused learning is a line of work wherein the decision outcomes are directly optimized rather than following a predict-then-optimize framework. Different kinds of one-shot \cite{donti2017task,perrault2020end,wilder2019melding} and sequential optimization problems ~\cite{wang2021learning,futoma2020popcorn} can be solved end-to-end by blending the decision outcome into the downstream optimization problem. In \cite{wang2022decision}, a decision focused learning framework is proposed for RMABs, where transition dynamics are learnt by directly optimizing the final decision outcome using off-policy policy evaluation (OPE).  Unfortunately, OPE with limited data is often not very stable and requires extensive tuning to get desired results \cite{huang2020importance}. Moreover such an end-to-end optimization results in low interpretability of the results. There are several differences between this line of work and ours. We focus on real-world deployed system to illustrate that improved prediction accuracy using standard error metrics may not result in improved overall decision quality. In addition we focus on RMABs and provide tailored approaches to evaluate and explain the performance of the prediction component of RMABs.

% \citet{arpitaijcai, avrachenkov2020whittle}, present a Whittle Index-based Q-learning approach for unknown RMAB parameters. However, their techniques either assume identical arms or rely on receiving thousands of samples from each arm, which is unrealistic in our setting, given limited overall stay of a beneficiary in an information program --- a beneficiary may drop out or stop engaging with the program few weeks post enrolment unless a service call convinces them to do otherwise. Instead, we present a novel approach that applies clustering to the available historical data to infer model parameters.


% Clustering in the context of Multi-Armed Bandit and Contextual Bandits has received significant attention in the past \cite{gentile2014online,li2019improved, yang2020exploring,li2021unifying}, but these settings do not consider restless bandit problems. \cite{mintz2020nonstationary} tackles a non-stationary setup with stochastic rewards, 
% %that is simplified using sleeping states in our method 
% while \cite{ayer2019prioritizing} infers model parameters from independent studies in absence of historic data. In contrast, we focus on learning RMAB parameters using clustered historic beneficiary data. \cite{zhou2018personalizing, liao2020personalized} propose building predictive models per beneficiary in an online fashion, which is infeasible in our setup given the short stay of the beneficiaries.


==> AI4SG Workshop (AAAI 23) Submission/transition_probability_error_analysis.tex <==
\section{Analyzing Errors in the Prediction Stage}% [Paritosh]}
\label{section:transition_probability_errors}

In this section, we provide a comparative analysis of the performance of the RMAB system in the three field tests and we highlight the key learning from these studies. We begin by analyzing the errors in predicting transition probabilities. The main observation we make here is that an overall improvement in the prediction accuracy -- at least as measured by standard metrics such as RMSE or MEA -- may not result in a concomitant improvement in the real-world performance. %Therefore, analyzing the system's performance based on just the prediction accuracy is insufficient and reducing errors in prediction accuracy may not guarantee a performance improvement.

\subsubsection{Comparing Prediction Errors across Studies}
The RMAB-based system in its first phase predicts the MDP parameters of each arm, i.e., the transition probabilities for each beneficiary, denoted by $P_i(s,a,s')$ for each beneficiary $i$ and $s,a,s' \in \{0,1\}$. %The prediction of transition probabilities is based on the socio-demographic features of the beneficiaries -- this being the only data that is available for each beneficiary prior to a study/field test. However, during the study/field test we get to observe the actual behaviours of the beneficiaries which are based on their \emph{true} or observed transition probabilities. Thus, at the end of the study we can empirically estimate the true transition probabilities of each beneficiary. To gauge the performance of our RMAB system in the prediction phase, 
We define the prediction error based on comparing the predicted transition probabilities and the observed transition probabilities for each beneficiary.  We use $O_i(s,a,s')$ to denote the observed (or true) transition probability for each beneficiary. %However, this analysis can be performed in different ways which complement each other.
%We now present the analysis of prediction accuracy across the different studies. % This analysis is divided into three parts (a) analysis of cumulative prediction errors, (b) errors in computing each transition probability, (i.e., transition probability-wise prediction errors), and (c) comparing the distributions of the predicted vs observed transition probabilities.
% \subsection{Cumulative transition probability prediction errors}
Note that, the transition probabilities corresponding to each beneficiary are related by the equations $P_i(s,a,s') = 1 - P_i(s,a, 1-s')$ and $O_i(s,a,s') = 1 - O_i(s,a, 1-s')$ for each  $s,a,s' \in \{1,0\}$. We take this fact into consideration while defining the cumulative error for each beneficiary, the definition of cumulative error is based on only the four independent transition probabilities $P_i(s, a, s)$ where $s,a \in \{0,1\}$.

There are two natural ways of defining the cumulative errors of each beneficiary $i$: first, as the Root Mean-Square Error (RMSE) denoted by $\mathcal{E}_i^{RMSE}$ and second as the Mean Absolute Error (MAE) denoted by $\mathcal{E}_i^{MAE}$. Formally,

\begin{align*}
    \label{equation:cumulative_errors}
    \mathcal{E}^{RMSE}_i = \sqrt{\frac{1}{4} \sum_{s \in \{0,1\}} \sum_{a \in \{0,1\}} \big(P_i(s,a,s) - O_i(s,a,s)\big)^2}
\end{align*}

\begin{align*}
    % \label{equation_MAE_error}
    \mathcal{E}^{MAE}_i = \frac{1}{4} \sum_{s \in \{0,1\}} \sum_{a \in \{0,1\}} |P_i(s,a,s) - O_i(s,a,s)|
\end{align*}

% Simply stated, the cumulative error $\mathcal{E}^c_i$ is the RMSE error computed between the four independent predicted probabilities $\langle P_i(s, a, s)\rangle_{s,a \in \{0,1\}}$ and observed probabilities $\langle O_i(s, a, s) \rangle_{s,a \in \{0,1\}}$. 
For each beneficiary, we compute the cumulative error values --- $\mathcal{E}^{RMSE}_i$ and $\mathcal{E}^{MAE}_i$ --- as defined above. We then compare the distribution of cumulative errors, and analyze the mean and median error values across the three studies we performed.

\begin{table}[!htbp]
\centering
\caption{Cumulative transition probability prediction errors across studies.}\label{table:cumulative-tp-errors}
\begin{tabular}{|c|c|c|c|}
 \hline
 Error statistics & Apr 2021 & Jan 2022 &  May 2022 \\ 
 \hline \hline
 %Mean of cumulative RMSE error
 Mean of $\mathcal{E}^{RMSE}_i$ & 0.382 & 0.451 & 0.345 \\ 
 Median of $\mathcal{E}^{RMSE}_i$ & 0.375 & 0.461 & 0.340 \\
 Mean of $\mathcal{E}^{MAE}_i$ & 0.333 & 0.4 & 0.3 \\ 
 Median of $\mathcal{E}^{MAE}_i$ & 0.311 & 0.394 & 0.291 \\
 \hline


 
%  ./Study1:may20-apr21/: mean MAE = 0.333, median MAE = 0.311
% ./Study3:apr21-jan22/: mean MAE = 0.4, median MAE = 0.394
% ./Study5:Jan22-May22/: mean MAE = 0.3, median MAE = 0.291
%  Mean error for $(E, p, E)$ & 0.441 & 0.448 & 0.326 \\ 
%  Median error for $(E, p, E)$ & 0.425 & 0.479 & 0.272 \\
% \hline
%  Mean error for $(E, a, E)$ & 0.351 & 0.448 & 0.291 \\ 
%  Median error for $(E, a, E)$ & 0.323 & 0.435 & 0.218 \\
% \hline
%  Mean error for $(NE, a, NE)$ & 0.278 & 0.31 & 0.298 \\ 
%  Median error for $(NE, a, NE)$ & 0.22 & 0.25 & 0.261 \\
% \hline
%  Mean error for $(NE, p, NE)$ & 0.261 & 0.354 & 0.287 \\ 
%  Median error for $(NE, p, NE)$ & 0.217 & 0.363 & 0.243 \\
%  \hline
\end{tabular}
\end{table}

In Table \ref{table:cumulative-tp-errors} the mean and the median of cumulative errors, $\mathcal{E}^{RMSE}_i$ and $\mathcal{E}^{MAE}_i$, are shown for the three field studies; the mean and median is computed across all the beneficiaries. Clearly, we can see that the errors in January 2022 study are the highest, wrt to both mean and median. In fact, the cumulative errors are in the following order: errors in January 2022 are the highest, followed by April 2021, and the lowest prediction errors are observed in May 22 study. 

Indeed, this is in direct contrast with the real-world performance of RMAB observed in these studies: as previously illustrated, the performance of RMAB system in May 2022 was much worse as compared to April 2021. Thus, the prediction accuracy, measured by using the standard measures like RMSE and MAE, are not at all indicative of the real-world performance of the RMAB system.

\begin{figure}[!htbp]
\centering
\includegraphics[width=0.8\columnwidth]{cumulative_tp_error_comparison.png}
\caption{The cumulative errors distribution in January 2022 is skewed towards the high-error region, whereas in May 2022 the errors are localized in the low-error region.} \label{figure:cumulative_tp_errors}
\end{figure}

To get more insight, in addition to comparing the mean and median error values, we also analyze the distribution of error values. The distribution of cumulative RMSE errors is shown in Figure \ref{figure:cumulative_tp_errors}. The error distributions, represented as violin plots, depicts the error distribution as a density function. Specifically, error values are shown on the y-axis and the x-axis shows the error density --- the higher the error density for a particular error value, the higher the width of the violin plot at the particular error value\footnote{Since distributions are represented by density function, the area under each distribution is the same}.

Clearly, the distribution of errors is more spread apart in January 2022 -- the errors are concentrated in the high-error regions (error values 0.4 and above). In contrast, the error distribution for the May 2022 study is localized in the low-error region and the distribution tapers in the high-error region (error values 0.5 and above). For the April 2021 study, we can observe two bumps in the error distribution, first, around the error density 0.6 and second around the error density 0.4; the bump in the high-error region is causing the mean and median error values to become higher. Thus, upon visually comparing the error distribution, we arrive at the same conclusion: the prediction errors in January 2022 are the highest, the errors are the lowest in May 2022 study and in April 2021 the errors lie in between the other two studies. Again this is in direct contrast with the performance of the RMAB system in these studies as depicted in Figure \ref{fig:studies} where we see that the performance of RMAB in May 2022 was worse as compared to April 2021.\\

% \subsection{Transition probability-wise prediction errors}
% To get a fine-grained perspective, we can also analyze the errors in computing each transition probability. Without loss of generality, we will only consider the four independent transition probabilities in this analysis, i.e., the probabilities $\langle P(s, b, s) \rangle$ for each state $s \in \{0,1\}$ and action $b \in \{0, 1\}$.

% For the transition probability $P(s, b, s)$ where $s,b \in \{0,1\}$, we define the error value in computing probability $P(s, b, s)$ for each beneficiary $i$ as the absolute value of the difference between the predicted and the observed transition probability, i.e., 

% \begin{align*}
% \mathcal{E}_i^{s,b,s} = |P_i(s,b,s) - O(s,b,s)|
% \end{align*}

% \noindent
% \emph{{\bf Part (a):} Errors in predicting probability of transition $(E, p, E)$}. The plots in the figure \ref{figure:tp_error_EpE} depict the distribution of errors in predicting the probability for transition $(E,p,E)$, i.e., $\mathcal{E}_i^{1,0,1}$ for all the three studies.\\

% \begin{figure}[!htbp]
% \centering
% \includegraphics[width=0.5\textwidth]{tp_error_E,p,E_comparison.png}
% \caption{The error distribution for transition $(E,p,E)$ is shown above. The errors in May 2022 are the lowest and they are highest in January 2022.} \label{figure:tp_error_EpE}
% \end{figure}

% % \begin{table}[!htbp]
% % \centering
% % \caption{Errors in predicting the probability of transition $(E, p, E)$ across studies.}\label{table:EpE-tp-errors}
% % \begin{tabular}{|p{5cm}|c|c|c|}
% %  \hline
% %  Error statistics for computing $(E, p, E)$ probability & April 2021 & January 2022 &  May 2022 \\ 
% %  \hline \hline
% %  Mean error & 0.441 & 0.448 & 0.326 \\ 
% %  Median error & 0.425 & 0.479 & 0.272 \\
% %  \hline
% % \end{tabular}
% % \end{table}

% We can see from table \ref{table:cumulative-tp-errors} that the errors in predicting transition probability for $(E,p,E)$ follow the same order as the cumulative errors -- the mean and median errors are the highest for the January 2022 study, followed by the April 2022 study, and they are the lowest for the May 2022 study.\\


% \noindent
% \emph{{\bf Part (b):} Error in predicting probability of transition $(E, a, E)$}. The distribution of errors in predicting the probability for transition $(E,p,E)$ , $\mathcal{E}_i^{1,0,1}$ are shown in fig \ref{figure:tp_error_EaE} and the corresponding values of mean and median errors is shown in table \ref{table:cumulative-tp-errors}. Here as well we observe that the errors in the May 2022 study are the lowest and the errors are highest in the January 2022 study.


% \begin{figure}[!htbp]
% \centering
% \includegraphics[width=0.5\textwidth]{tp_error_E,a,E_comparison.png}
% \caption{This distribution of errors in predicting the probability of transition $(E, a, E)$ is shown for all three studies.} \label{figure:tp_error_EaE}
% \end{figure}

% % \begin{table}[!htbp]
% % \centering
% % \caption{Errors in predicting the probability of transition $(E, a, E)$ across studies.}\label{table:EaE-tp-errors}
% % \begin{tabular}{|p{5cm}|c|c|c|}
% %  \hline
% %  Error statistics for computing $(E, a, E)$ probability & April 2021 & January 2022 &  May 2022 \\ 
% %  \hline \hline
% %  Mean error & 0.351 & 0.448 & 0.291 \\ 
% %  Median error & 0.323 & 0.435 & 0.218 \\
% %  \hline
% % \end{tabular}
% % \end{table}

% Next we examine the errors in computing transition probabilities for transitions in which the starting state is $NE$, i.e., the transitions $(NE, a, NE)$ and $(NE, p, NE)$.\\


% \noindent
% \emph{{\bf Part (c):} Error in predicting probability of transition $(NE, a, NE)$}.\\
% Figure \ref{figure:tp_error_NEaNE} shows the distribution of errors in predicting the probability of transition $(NE, a, NE)$ (i.e., the distribution of $\mathcal{E}_i^{0,1,0}$) for all three studies. The corresponding values of mean and median error are detailed in table \ref{table:cumulative-tp-errors}.

% \begin{figure}[!htbp]
% \centering
% \includegraphics[width=0.5\textwidth]{tp_error_NE,a,NE_comparison.png}
% \caption{This distribution of errors in predicting the probability of transition $(E, a, E)$ is shown for all three studies.} \label{figure:tp_error_NEaNE}
% \end{figure}

% % \begin{table}[!htbp]
% % \centering
% % \caption{Errors in predicting the probability of transition $(NE, a, NE)$ across studies.}\label{table:NEaNE-tp-errors}
% % \begin{tabular}{|p{5cm}|c|c|c|}
% %  \hline
% %  Error statistics for computing $(NE, a, NE)$ probability & April 2021 & January 2022 &  May 2022 \\ 
% %  \hline \hline
% %  Mean error & 0.278 & 0.31 & 0.298 \\ 
% %  Median error & 0.22 & 0.25 & 0.261 \\
% %  \hline
% % \end{tabular}
% % \end{table}

% We can see that the errors no longer follow the order of the cumulative predictive errors -- the mean and median of error values $\mathcal{E}_i^{0,1,0}$ for May 2022 study are not the lowest. In fact, the errors are highest in January 2022 study, followed by May 2022 and the errors are the lowest in Apr 2021 study.\\

% \noindent
% \emph{{\bf Part (d):} Error in predicting probability of transition $(NE, p, NE)$}.\\
% A similar pattern is observed for the errors in computing transition probability for $(NE, p, NE)$; distribution of these errors are shown in fig \ref{table:cumulative-tp-errors}. Particularly, from \ref{table:cumulative-tp-errors} we can see that the errors are highest in January 2022, followed by May 2022, and the errors are the lowest in April 2021 study. Indeed, the errors $\mathcal{E}_i^{0,0,0}$ do not follow the order of the cumulative errors, specifically, the errors in May 2022 study are not the lowest wrt both mean and median errors.

% \begin{figure}[!htbp]
% \centering
% \includegraphics[width=0.5\textwidth]{tp_error_NE,p,NE_comparison.png}
% \caption{This distribution of errors in predicting the probability of transition $(NE, p, NE)$ is shown for all three studies.} \label{figure:tp_error_NEpNE}
% \end{figure}

% % \begin{table}[!htbp]
% % \centering
% % \caption{Errors in predicting the probability of transition $(NE, p, NE)$ across studies.}\label{table:NEpNE-tp-errors}
% % \begin{tabular}{|p{5cm}|c|c|c|}
% %  \hline
% %  Error statistics for computing $(NE, p, NE)$ probability & April 2021 & January 2022 &  May 2022 \\ 
% %  \hline \hline
% %  Mean error & 0.261 & 0.354 & 0.287 \\ 
% %  Median error & 0.217 & 0.363 & 0.243 \\
% %  \hline
% % \end{tabular}
% % \end{table}

% % \subsection{Comparing Distributions of Predicted and Observed Transition Probabilities}
% % Next we plot and compare, for each of the four independent transition probabilities, (i) the distribution of the predicted transition probability for the entire population of the beneficiaries with (ii) the distribution of the observed transition probabilities for the entire population of the beneficiaries. %These distributions can be compared side-by-side comparison for all the three studies. 
% % Figure \ref{figure:prob_distribution_comparison} depicts this comparison of the distributions of the predicted vs the observed probabilities.

% % \begin{figure}[!htbp]
% % \centering
% % \includegraphics[width=\textwidth]{probability_distribution_comparision.png}
% % \caption{A side-by-side comparison of the probability distribution of the predicted and observed transition probabilities is shown for all three studies.} \label{figure:prob_distribution_comparison}
% % \end{figure}

% % From figure \ref{figure:prob_distribution_comparison} we can observe that the distribution of predicted probabilities and observed probabilities are very similar for the May 22 study compared to other studies. This explains the lower values of cumulative errors in May 22. Additionally, the distribution of predicted and observed probabilities do not match for the January 2022 study, which supports the fact that cumulative errors were the highest in that study.




==> AI4SG Workshop (AAAI 23) Submission/whittle_index_error_analysis.tex <==
\section{Decision-Focused Evaluation: Analysing Errors in Computing Whittle Indices}% [Paritosh]}
\label{section:decision_focused_analysis}

%In the prediction accuracy analysis detailed in the previous section we saw that the errors in the May 22 study are the lowest. However, as we saw in Section \ref{section:previous_studies}, our RMAB-based system did not perform well in the May 22 study. In fact, the performance of RMAB system was significantly worse than the April 2022 study, which is in complete dissonance with the fact that cumulative errors in May 2022 are lower than April 2021. Thus, the errors in prediction accuracy are not a good predictor of the real-world performance. 

We now present the decision-focused criterion for analyzing the performance of RMABs. The central idea behind decision-focused evaluation is to analyze the errors in the final decision quality which in turn is captured by the Whittle indices in our formulation. Indeed, this analysis is much more aligned with the Whittle index policy for solving RMABs, as it reveals how inaccurate the RMAB system was in predicting the top Whittle indices.

At every decision step (i.e., every week for ARMMAN), the Whittle index policy selects k beneficiaries having the highest Whittle index (as per their current states). Given this, it is natural to perform the Whittle index error analysis week-by-week. Specifically, for a given study and a given week, we analyze the errors in computing top-k Whittle indices. %After intervening these k beneficiaries, the state of every beneficiary updates and thus their Whittle indices are also different in the next state. Notably here the Whittle indices are computed based on the predicted transition probabilities, thus we will refer them as predicted Whittle indices.

To compute the Whittle index errors, we compare the top-k predicted Whittle indices of beneficiaries to the \emph{observed Whittle indices} -- the Whittle indices of beneficiaries computed using the observed (true) transition probabilities. %In other words, we will consider the Whittle indices computed using the observed transition probabilities as the ground truth or baseline of comparison for defining the error. Indeed, the observed transition probabilities capture the true behavior of the beneficiaries therefore the Whittle indices based on observed probabilities i.e., observed Whittle indices are the indices based on which our RMAB system should have selected beneficiaries for intervention.

We begin by introducing required notations. For simplicity, we will use the set of first n natural numbers $[n] = \{1, 2, \ldots, n\}$ to denote the set of all beneficiaries; here $n$ denotes the total number of beneficiaries. For a given week, we will use a permutation $P = (b_1, b_2, \ldots, b_n)$ of $[n]$ to denote the ordered sequence of beneficiaries sorted in descending order as per their Whittle indices. %Note that, in a given week, every beneficiary is in a particular state and corresponding to that state there is a associated Whittle index, permutation $P$ orders beneficiaries as per this Whittle index in descending order. 
Similarly, we define $O = (b'_1, b'_2, \ldots, b'_n)$ to denote the ordering of beneficiaries as per their observed Whittle indices in descending order, i.e., $b'_1$ has the highest observed Whittle index in a given week. Furthermore, the integers $\{1, 2, 3, \ldots, k\}$ will be used to denote the $k$ beneficiaries having the highest predicted Whittle indices in a given week, i.e., beneficiary $i$ has the the $i$th highest Whittle index in that week.

% We compare and contrast different ways of defining Whittle index errors and show that a definition based on a modification of Spearman's footrule is best suited for RMAB-based systems.


\subsection{Quantifying errors in top-k Whittle indices}

Errors in top Whittle indices can be defined in multiple ways and apriori it is not clear which method is the most appropriate. We next present a comparative analysis of various definitions of errors in top-k Whittle indices. We begin by highlighting the shortcomings of the seemingly-natural ways of defining the errors in top-k Whittle indices. Based on this, we select an error definition that doesn't suffer from these shortcomings and we use it to analyze the errors in top-k Whittle indices across the three studies.\\

\noindent
\emph{{\bf 1. Absolute and Normalized Whittle Index Errors:}} Denote by $WI_i^p$ and $WI_i^o$ the predicted and observed Whittle indices of each beneficiary $i$ having top-k predicted Whittle index in a given week i.e. $i \in \{1, 2, \ldots, k\}$. Given this, arguably the simplest way of defining errors in top-k Whittle index is to consider the absolute difference in the predicted and the observed Whittle index for all top-k beneficiaries, denoted by $\mathcal{E}^{abs} = \frac{1}{k} \sum_{i=1}^k |WI^p_i - WI^o_i|$.
However, this seemingly natural definition of errors has an issue: the error values cannot be compared between different studies or different algorithms because the predicted \& observed Whittle indices between two studies can have very different magnitudes as they depend on the cohort of beneficiary in a study; see appendix for supporting data. To mitigate this we can define the normalized error value of each beneficiary $i$ so that it captures the percentage change between the predicted Whittle indices and the observed Whittle indices. 
Formally,

\begin{align*}
    \mathcal{E}^{norm} = \frac{1}{k} \sum_{i=1}^k \frac{|WI^p_i - WI^o_i|}{|WI^p_i|}
\end{align*}

However, this error definition also suffers from a similar issue. We observe that the normalization factor in the denominator i.e., the predicted Whittle indices, $WI^p_i$, depend on the cohort of the beneficiaries, and vary a lot in their magnitudes for different studies, making the error values incomparable across different studies; the details of this observation been deferred to the Appendix.

Notably, a high level issue with both the previous two definitions is that the error values depends on the magnitude of the Whittle indices and not on the ordering, while the Whittle index policy takes decisions solely based on the ordering of Whittle indices. This motivates the use of more sophisticated error definitions that primarily depend on the Whittle index ordering.

%This issue is highlighted through the following example: consider the case when the the predicted Whittle index of every beneficiary is twice the value of the observed Whittle index in a way that the ordering $P$ is exactly same as the ordering $O$. In such a case, the error values would be non-zero, however, since the ordered sequence $P$ is same as $O$, the Whittle index policy will select exactly those beneficiaries which would have been selected if decisions were made on the basis of observed Whittle indices -- the error should have been zero. Next we look at such definitions.\\

\noindent
\emph{{\bf 2. Kendall Tau distance for top-k:}} 
The Kendall Tau distance\cite{diaconis1977spearman} is a well-known metric for quantifying disarray between two permutations. For a given permutation $\pi$, denote by $\pi(i)$ the rank or the index of element $i \in [n]$ in the permutation $\pi$. Let $\sigma$ and $\pi$ be two permutations of the same set of element $[n] = \{1, 2, \ldots, n\}$.  The Kendall Tau distance between $\sigma$ and $\pi$, $\mathcal{K}(\sigma, \pi)$, is defined to be the fraction of discordant pairs between the two permutations, i.e., $\mathcal{K}(\sigma, \tau) = 2/n(n-1) \sum_{1 \leq i < j \leq n} \overline{\mathcal{K}}_{i,j}(\sigma, \tau)$ where $\overline{\mathcal{K}}_{i,j}(\sigma, \tau) = 1$ if the elements $i$ and $j$ are in the same order in both permutations $\sigma$ and $\pi$ and $\overline{\mathcal{K}}_{i,j}(\sigma, \tau) = 0$ otherwise. Formally, $\overline{\mathcal{K}}_{i,j}(\sigma, \pi) = (\sigma(i) > \sigma(j) \land \pi(i) < \pi(j)) \lor (\sigma(i) < \sigma(j) \land \pi(i) > \pi(j))$.

Note that, the Kendall Tau distance quantifies the disarray between relative ordering of elements in two permutations. %However, for capturing the errors in computing top Whittle indices we only want to consider the disarray between (i) the top-k elements of the ordering $P$ and (ii) the same elements in the ordering $O$. %This is because the Whittle index policy selects the top-k beneficiaries as per the predicted Whittle indices. 
To suit our context, we can modify it to capture the disarray in the top-k elements of $P$, we call this metric the top-k Kendall Tau distance, $\mathcal{K}^{top-k}(\sigma, \tau)$. Let $(s_1, s_2, \ldots, s_k)$ be the top-k elements in the permutation $\sigma$. Given this, the top-k Kendall Tau distance is defined as 

\begin{align*}
    \mathcal{K}^{top-k}(\sigma, \tau) = \frac{2}{n(n-1)} \sum_{1 \leq i < j \leq k} \overline{\mathcal{K}}_{s_i,s_j}(\sigma, \tau)
\end{align*}

where $\sigma$ and $\tau$ are permutations on $k$ elements \footnote{Note that unlike the normalized Kendall Tau distance, the top-k Kendall Tau distance is not symmetric, i.e., $\mathcal{K}^{top-k}(\sigma, \pi) \neq \mathcal{K}^{top-k}(\sigma, \pi)$.}. Based on this definition, we define the errors in top-k Whittle indices as $\mathcal{E}^{kt} = \mathcal{K}^{top-k}(P, O)$. While this error value $\mathcal{E}^{kt}$ can be compared across different studies and different weeks of a given study (because it is normalized by $n(n-1)/2$ and the error values do not depend on the magnitude of Whittle indices), the error definition still has an issue: consider the case when the top-k elements of $P$ appear in the same relative order at the end of the permutation $O$ (i.e., as a suffix); the error value, $\mathcal{E}^{kt} = 0$ for this case. However, in this case, we would want the error to be high since the beneficiaries predicted to have the top-k Whittle indices actually have the lowest observed Whittle indices. In other words, this error definition only captures the relative difference between the ordering of the top-k elements in the orderings $P$ and $O$ -- ignoring their relative positions -- whereas, as highlighted by the previous example, this is insufficient to semantically quantify the Whittle index errors.\\

\noindent
\emph{{\bf 3. Spearman's footrule for top-k:}} We now present a definition of errors in top-k Whittle indices that is a modification of the well-known Spearman's footrule distance \cite{diaconis1977spearman} used to quantify the difference between two permutations. We then show that this definition does not suffer from the shortcomings of the previous definition, and finally compare the errors across different studies wrt this decision-focused error definition. Formally, the Spearman's distance $\mathcal{S}(\sigma, \pi)$ between two permutations $\sigma$ and $\pi$ of the set $[n] = \{1, 2, \ldots, n\}$ is defined as $\mathcal{S}(\sigma, \pi) = \sum_{i=1}^n |\sigma(i) - \pi(i)|$.

To capture the errors in top-k Whittle indices we modify the Spearman's footrule to $(i)$ consider only the top-k elements in $\sigma$ and additionally $(ii)$ we add a normalization factor of $n$. Without loss of generality, let $(s_1, ,s_2 \ldots, s_k)$ be the top-k elements of $\sigma$. Then, the Spearman's footrule for top-k is defined as

\begin{align*}
    \mathcal{S}^{top-k}(\sigma, \pi) & = \frac{1}{k} \sum_{i=1}^k \frac{|\sigma(s_i) - \pi(s_i)|}{n} = \frac{1}{k} \sum_{i=1}^k \frac{|i - \pi(s_i)|}{n} \tag{since $\sigma(s_i) = i$}
\end{align*}

The normalization factor of $n$ is added to the denominator because the quantity $|\sigma(i) - \pi(i)|$ is bounded by the total number of elements/beneficiaries $n$ --- after normalization the error values lie in the interval $[0,1]$ enabling comparison of error values across different studies wherein the number of beneficiaries, $n$, are different. Based on this definition, we define the error in top-k Whittle indices as $\mathcal{E}^{s} = \mathcal{S}^{top-k}(P, O) = \frac{1}{k} \sum_{i=1}^k \frac{|i - O(s_i)|}{n}$ where $s_1, s_2, \ldots, s_k$ are the first $k$ elements of $P$. Additionally, the Whittle index error for each beneficiary $i$ having rank $i$ as per the predicted Whittle index will be denoted by $\mathcal{E}^s_i = \frac{|i - O(s_i)|}{n}$. Therefore,

\begin{align}
    \label{definition:Spearman-WI-error}
    \mathcal{E}^s = \frac{1}{k} \sum_{i=1}^k \mathcal{E}^s_i \ \ \text{ where } 1 \leq i \leq k, \ \ \mathcal{E}^s_i = \frac{|i - O(s_i)|}{n}
\end{align}

This definition quantifies the average shift in the ranks/indices of the top-k beneficiaries (as per ordering $P$) between $P$ and $O$ --- intuitively this is the quantity we want to capture in the error value as the decisions made by RMAB system as based on top-k Whittle indices. Indeed this error definition does not depend on the Whittle index magnitudes and does not suffer from the shortcomings of the previous definitions. 

In the next section, we show that the error values based on the top-k Spearman's footrule distance for the three studies indeed match-up perfectly with the performance of the RMAB-based system observed in the real-world.

\subsection{Errors in Computing top-k Whittle indices}

%In this section, we analyze the errors in computing the top Whittle indices for the three real-world studies. 
As previously described, we use the error definition based on the top-k Spearman's footrule, $\mathcal{E}^s = \mathcal{S}^{top-k}(P, O) = \frac{1}{k} \sum_{i=1}^k \frac{|i - O(i)|}{n}$. 


For the three studies we compare the errors in top-200 Whittle indices, i.e., we set $k= 200$. This choice is based on the fact that the number of interventions in the April 2021, January 2022, and May 2022 studies are 125, 250, and 175 respectively. Therefore, the value $k = 200$ acts as a middle-ground, enabling fair comparison across studies.

First we will compare the Whittle index error values across the studies, week-by-week, for the first four weeks of all the studies. Then, we will analyze the cumulative errors which combine the weekly error values into a single per-study error value.\\

\noindent
\emph{{\bf (i) Week-by-week comparison of Whittle index errors:}} The mean and median values of the Whittle index errors for the first four weeks of each study are shown in tables \ref{table:mean-WI-errors}, \ref{table:median-WI-errors} respectively.

\begin{table}[!htbp]
\centering
\caption{Week-wise comparison of mean errors in computing top Whittle indices.}\label{table:mean-WI-errors}
\begin{tabular}{|p{2.5cm}|c|c|c|}
 \hline
 Week of the study & Apr 2021 & Jan 2022 &  May 2022 \\ 
 \hline \hline
 Week 1 & 0.424 & 0.505 & 0.492 \\ 
 Week 2 & 0.439 & 0.486 & 0.495 \\ 
 Week 3 & 0.435 & 0.488 & 0.49 \\ 
 Week 4 & 0.446 & 0.502 & 0.465 \\
 \hline
 Cumulative mean errors & 0.436 & 0.495 & 0.486 \\
 \hline
\end{tabular}
\end{table}

\begin{table}[!htbp]
\centering
\caption{Week-wise comparison of median errors in computing top Whittle indices.}\label{table:median-WI-errors}
\begin{tabular}{|p{2.5cm}|c|c|c|}
 \hline
 Week of the study & Apr 2021 & Jan 2022 &  May 2022 \\ 
 \hline \hline
 Week 1 & 0.376 & 0.481 & 0.471 \\ 
 Week 2 & 0.387 & 0.468 & 0.488 \\ 
 Week 3 & 0.389 & 0.485 & 0.477 \\ 
 Week 4 & 0.396 & 0.473 & 0.46 \\
 \hline
 Cumulative median errors & 0.387 & 0.477 & 0.473 \\
 \hline
\end{tabular}
\end{table}

We can observe that the Whittle index error values are the highest for the January 2022 study, followed by May 2022 study and they are the lowest for the April 2021 study. This order of the error values exactly match with the real-world performance of the RMAB system in these studies (Figure \ref{fig:studies}) where the performance of RMAB systems was best in April 2021, followed by May 2022, and January 2022. Therefore, unlike the prediction accuracy analysis, the errors in top-k Whittle indices --- the decision-focused evaluation criterion --- is able to explain the overall performance of the RMAB system in the real-world. In principle, this makes sense because the RMAB system uses top-k Whittle indices to take intervention decisions, while transition probabilities are essentially intermediate values that do not directly influence the decision choices made by RMAB system. \\

\noindent
\emph{{\bf (ii) Comparison of cumulative Whittle index errors:}}
In addition to comparing the errors week-by-week, we can combine the error values across all four weeks for each study to get a per-study error distribution. This distribution of errors is shown in Figure \ref{figure:WI_error_distribution}. Tables \ref{table:mean-WI-errors} and \ref{table:median-WI-errors} list the corresponding values of cumulative mean and median errors. Here also we observe that the errors in April 2021 are lower as compared to the other studies.

\begin{figure}[!htbp]
\centering
\includegraphics[width=0.8\columnwidth]{cumulative_WI_errors.png}
\caption{The distribution of top-k Whittle index errors is shown for all three studies.} \label{figure:WI_error_distribution}
\end{figure}

\section{Probabilistic Analysis: Comparing RMAB System to a Purely Random Algorithm}
\label{appendix:probabilistic-analaysis}
To theoretically explain the varying performance of RMAB across studies we present a comparison between the RMAB system and a \emph{purely random algorithm} -- an algorithm which selects $k$ beneficiaries uniformly at random (with replacement) for intervention every week -- based on a probabilistic analysis. The analysis is based on computing the expected value and variance of the Whittle index error $\mathcal{E}^s$ (equation \ref{definition:Spearman-WI-error}) for a purely random algorithm. The resulting error values are then used as a baseline to compare the Whittle index error values observed in all the three studies. Thus, this analysis can be interpreted as answering the question: \emph{how well did the RMAB-based system perform as compared to the purely random algorithm?} Due to space limitation the entire analysis has been deferred to the Appendix.




==> problem_statement.tex <==
\section{Problem Statement}% [Paritosh and Shresth]}

Our aim is to understand how prediction accuracy relates to the overall performance of a deployed RMAB system. This understanding is required to guide system improvements and is crucial for monitoring, diagnosing, and interpreting the performance of deployed RMAB system. One might expect to see improvement in performance following an improvement in prediction accuracy, thus prediction accuracy might seem to be a natural objective to steer the design of the overall RMAB system.

However, we show that simply improving the prediction accuracy for RMABs may not result in overall performance improvement, and therefore an alternate evaluation method is needed for RMAB systems. Moreover, there are multiple, seemingly-reasonable ways in which we can evaluate RMAB systems, and it is not immediately clear which is the most appropriate criterion. Consequently, our goal is to design a method of evaluating RMAB systems that correlates with and offers insights into the real-world performance, and additionally is versatile enough to enable analysis from various perspectives.


% This is motivated by the fact that RMABs can be used to model a wide variety of sequential decision making problems in various domains like security, wildlife conservation, public health, etc. 



% such that the decrease in error also gets reflected in improvement in the real-world performance. 
% In this work, we propose such a definition of errors in top-k Whittle indices. Additionally, using probabilistic analysis we give bounds on the expectation and the standard deviation of this error value, so that we can quantify how much better is the RMAB system performing as compared to a purely random policy.
% We pose the question of understanding the relationship between prediction accuracy  and overall RMAB system performance. This is critical for two reasons: First, it is useful to understand the value of investing on improving predictive accuracy towards improving the final system performance. Second, this understanding is instructive in monitoring and diagnosing the performance of a deployed RMAB system.  

% Towards facilitating this understanding, our contributions are as follows. First we provide and analyze the results from a first-of-its-kind deployment of RMABs. Second we illustrate that, counter to natural expectations, improved overall prediction accuracy does not lead to improvement in  the real-world performance of the RMAB system. Third, we present a decision-focused evaluation approach of the predictive component and show that it is better at explaining the performance of real-world RMAB system. Fourth we propose specific decision-focused evaluation metrics, which we hope would guide diagnosis of RMAB systems in the future.
